Robust Reinforcement Learning for Continuous Control with Model Misspecification

We provide a framework for incorporating robustness -- to perturbations in the transition dynamics which we refer to as model misspecification -- into continuous control Reinforcement Learning (RL) algorithms. We specifically focus on incorporating robustness into a state-of-the-art continuous control RL algorithm called Maximum a-posteriori Policy Optimization (MPO). We achieve this by learning a policy that optimizes for a worst case expected return objective and derive a corresponding robust entropy-regularized Bellman contraction operator. In addition, we introduce a less conservative, soft-robust, entropy-regularized objective with a corresponding Bellman operator. We show that both, robust and soft-robust policies, outperform their non-robust counterparts in nine Mujoco domains with environment perturbations. In addition, we show improved robust performance on a high-dimensional, simulated, dexterous robotic hand. Finally, we present multiple investigative experiments that provide a deeper insight into the robustness framework. This includes an adaptation to another continuous control RL algorithm as well as learning the uncertainty set from offline data. Performance videos can be found online at https://sites.google.com/view/robust-rl.

==> defs.tex <==
% Citing
\newcommand{\cp}{\citep}
\newcommand{\ca}{\citeauthor}
\newcommand{\cy}{\citeyear}
\newcommand{\ct}{\citet}
\newcommand{\ctp}[1]{\ca{#1}'s~(\cy{#1})}
\newcommand{\cwp}[1]{\ca{#1}, \cy{#1}}
\newcommand{\ctt}[1]{\ca{#1}~\cp{#1}} % this is to avoid [] in the next line

\newcommand{\mat}[1]{\ensuremath{\boldsymbol{\mathrm{#1}}}}
\newcommand{\fnc}[1]{\ensuremath{\mathrm{#1}}}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}

\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\M}{\ensuremath{\mathcal{M}^{\phi}}}
\newcommand{\MM}{\ensuremath{\mathcal{M}}} 
\newcommand{\CC}{\ensuremath{\mathcal{C}}} 
\newcommand{\E}{\ensuremath{\mathrm{E}}}
\newcommand{\MMtr}{\ensuremath{\hat{\MM}}} 
\newcommand{\Mtr}{\ensuremath{\hat{M}}}
\newcommand{\wtr}{\ensuremath{\hat{\mat{w}}}}
\newcommand{\rtr}{\ensuremath{\hat{r}}}
\newcommand{\rvtr}{\ensuremath{\hat{\mat{r}}}}
\newcommand{\Rtr}{\ensuremath{\hat{R}}}
\newcommand{\Wtr}{\ensuremath{\hat{\mat{W}}}}

\newcommand{\Normal}{\ensuremath{\mathcal{N}}}

\newcommand{\w}{\mat{w}}
\newcommand{\WW}{\mat{W}}
\newcommand{\Wt}{\ensuremath{\tilde{\mat{W}}}}
\renewcommand{\r}{\mat{r}}
\newcommand{\z}{\mat{z}}
\newcommand{\zw}{\mat{zw}}
\newcommand{\Z}{\mat{Z}}
\newcommand{\vphi}{\mat{\phi}}
\newcommand{\vpsi}{\mat{\psi}}
\newcommand{\vprm}{\mat{\z}}
\newcommand{\tvphi}{\ensuremath{\tilde{\mat{\phi}}}}
\newcommand{\tvpsi}{\ensuremath{\tilde{\mat{\psi}} }}
\newcommand{\tPsi}{\ensuremath{\tilde{\Psi} }}
\newcommand{\tmpsi}{\ensuremath{\tilde{\mat{\Psi}} }}
\newcommand{\MPhi}{\mat{\Phi}}
\newcommand{\MPsi}{\mat{\Psi}}
\renewcommand{\P}{\mat{P}}
\renewcommand{\t}{\ensuremath{\top}}



\renewcommand{\th}[1]{\text{#1$^\mathrm{th}$}}
\newcommand{\ith}{\th{i}}
\newcommand{\jth}{\th{j}}
\newcommand{\kth}{\th{k}}

\newcommand{\argmin}{\ensuremath{\mathrm{argmin}}}
\newcommand{\argmax}{\ensuremath{\mathrm{argmax}}}
\renewcommand{\min}{\ensuremath{\mathrm{min}}}

\newcommand{\Qmax}{\ensuremath{Q_{\mathrm{max}}}}
\newcommand{\pimax}{\ensuremath{\pi_{\max}}}
\newcommand{\Qpimax}{\ensuremath{Q^{\pi_{\max}}}}
\newcommand{\Tpimax}{\ensuremath{T^{\pi_{\max}}}}

\newcommand{\Mh}{\ensuremath{\hat{M}}} 
\newcommand{\Qh}{\ensuremath{\hat{Q}}}
\newcommand{\pih}{\ensuremath{\hat{\pi}}}
\newcommand{\wh}{\ensuremath{\hat{\w}}}
\newcommand{\Qhmax}{\ensuremath{\hat{Q}_{\mathrm{max}}}}
\newcommand{\pihmax}{\ensuremath{\pi}}
\newcommand{\Qhpimax}{\ensuremath{\hat{Q}^{\pi_{\max}}}}
\newcommand{\Thpimax}{\ensuremath{\hat{T}^{\pi_{\max}}}}

\newcommand{\rdif}{\ensuremath{\delta}}

\newcommand{\Qt}{\ensuremath{\tilde{Q}}}
\newcommand{\vQt}{\ensuremath{\tilde{\mat{Q}}}}
\newcommand{\pit}{\ensuremath{\tilde{\pi}}}
\newcommand{\Qtmax}{\ensuremath{\tilde{Q}_{\mathrm{max}}}}
\newcommand{\pitmax}{\ensuremath{{\pi}}}
\newcommand{\Qpitmax}{\ensuremath{Q^{\pi}}}
\newcommand{\Tpitmax}{\ensuremath{T^{\pi}}}
\newcommand{\wt}{\ensuremath{\tilde{\w}}}
\renewcommand{\H}{\mat{H}} 

\newcommand{\agt}{\fnc{agt}}

\newcommand{\piexp}{\ensuremath{\pi}}
\newcommand{\piexpj}{\ensuremath{_{\piexp_j}}}
\newcommand{\piexpi}{\ensuremath{_{\piexp_i}}}
\newcommand{\piexpk}{\ensuremath{_{\piexp_k}}}

\newcommand{\la}{\ensuremath{\leftarrow}}

\newcommand{\vpi}{\ensuremath{\mat{v}^{\pi}}}
\newcommand{\rpi}{\ensuremath{\mat{r}^{\pi}}}
\newcommand{\Ppi}{\ensuremath{\mat{P}^{\pi}}}

\newcommand{\phimax}{\ensuremath{\vphi_{\max}}}

\renewcommand{\S}{\ensuremath{\mathcal{S}}}
\newcommand{\A}{\ensuremath{\mathcal{A}}}
\newcommand{\W}{\ensuremath{\mathcal{W}}}

\newcommand{\score}{\ensuremath{\mathrm{score}}}
\newcommand{\currscore}{\ensuremath{\mathrm{curr\_score}}}
\newcommand{\ntpu}{\ensuremath{\mathrm{used}}}
\newcommand{\act}{\ensuremath{\mathrm{c}}}

\newcommand{\I}[1]{\ensuremath{\delta\{#1\}}} 
\newcommand{\II}{\ensuremath{\delta}} 

\newcommand{\vf}{\ensuremath{\mat{\varphi}}}
\newcommand{\vfi}{\ensuremath{\mat{\varphi}_i}}
\newcommand{\vfp}{\ensuremath{\mat{\varphi}_p}}
\newcommand{\vweights}{\mat{z}}
\newcommand{\od}{\ensuremath{\mat{o}}}
\newcommand{\rank}{\ensuremath{\mathrm{rank}}}

\newcommand{\ns}{\ensuremath{\mathrm{ns}}}
\newcommand{\nstr}{\ensuremath{n_{\mathrm{tr}}}}
\newcommand{\nsts}{\ensuremath{n_{\mathrm{ts}}}}
\newcommand{\dist}{\ensuremath{\mathcal{D}}}
\newcommand{\rt}{\ensuremath{\tilde{r}}}
\newcommand{\rvt}{\ensuremath{\tilde{\mat{r}}}}
\newcommand{\vrt}{\ensuremath{\tilde{\mat{r}}}}
\newcommand{\params}{\ensuremath{\mat{\theta}}}

\newcommand{\eb}{\ensuremath{\mathrm{extend\_basis}}}
\newcommand{\sfgpi}{SF\hspace{0.2mm}\&\hspace{0.2mm}GPI}
\newcommand{\sfgpirl}{\sfgpi\ continual}
\newcommand{\sfgpisl}{\sfgpi\ zero-shot}

\newcommand{\mo}{{\normalfont-{\tt 1}}}
\newcommand{\taskfive}{{\tt 1100}}
\newcommand{\tasksix}{{\tt 0111}}
\newcommand{\taskseven}{{\tt 1111}}
\newcommand{\taskeight}{{\tt \mo000}}
\newcommand{\tasknine}{{\tt \mo\mo00}}
\newcommand{\taskten}{{\tt \mo100}}
\newcommand{\taskeleven}{{\tt \mo1\mo0}}
\newcommand{\tasktwelve}{{\tt \mo101}}
\newcommand{\taskthirteen}{{\tt \mo1\mo1}}
\newcommand{\taskexample}{{\tt 1\mo00}}


\newcommand{\pitest}{\ensuremath{\pi_{\mathrm{test}}}}

\renewcommand{\dist}{\ensuremath{\mathcal{D}}}

\newcommand{\tderrorz}{\ensuremath{\mat{\delta}_{\z}^{t,n}}}
\newcommand{\tderrorwz}{\ensuremath{\mat{\delta}_{\w\z}^{t,n}}}
